Minimum Description Length Control

We propose a novel framework for multitask reinforcement learning based on the minimum description length (MDL) principle. In this approach, which we term MDL-control (MDL-C), the agent learns the common structure among the tasks with which it is faced and then distills it into a simpler representation which facilitates faster convergence and generalization to new tasks. In doing so, MDL-C naturally balances adaptation to each task with epistemic uncertainty about the task distribution. We motivate MDL-C via formal connections between the MDL principle and Bayesian inference, derive theoretical performance guarantees, and demonstrate MDL-C's empirical effectiveness on both discrete and high-dimensional continuous control tasks.

==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}
\RequirePackage{mathtools}

% use | for math mode
%\catcode`\|=3


% RL as inference
\newcommand{\opt}{\mathcal{O}}

% pg theory
\newcommand{\J}{\mathcal{J}^{\star}_\lambda}
\newcommand{\Jz}{\mathcal{J}^{\alpha}_\lambda}
\newcommand{\Ju}{\mathcal{J}_\lambda}
\newcommand{\kl}{\mathsf{KL}}
\newcommand{\pitheta}{\pi_{\theta}(a|s)}
\newcommand{\pistar}{\pi^*(a|s)}
\newcommand{\piz}{\pi_0}
\newcommand{\St}{\mathcal S}
\newcommand{\A}{\mathcal A}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\Dinf}{\left\| \frac{d_{\rho}^{\pi^\star} }{\mu}  \right \|_\infty}
\newcommand{\kappaA}{\kappa^\alpha_{\mathcal A}(s)}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\tv}{d_{\mathrm{TV}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathbb E}
\newcommand{\vw}{\vec w}
\newcommand{\prtr}{\mathsf P(s_{h+1}|s_h, a_h)}

% DRL
\newcommand{\Dq}{\stackrel{D}{=}}
\newcommand{\Dqdef}{\stackrel{D}{\coloneqq}}
\newcommand{\bellop}{\mathcal{T}}

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% symbols for probability distributions
\newcommand{\pr}{\mathsf{P}}
%\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
%\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
%\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lrset]{x} -> \mathbb{E}_a \lrset[ x \lrset]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lrset]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lrset]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lrset]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lrset]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
% \newcommand{\angles}[2][\lrset]{{\newlr #1\langle{#2}#1\rangle}}
\newcommand{\angles}[2][]{\lr[#1]\langle\rangle{#2}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lrset]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
%\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
%                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
%\newcommand{\KL}[3][]{\ensuremath{\textbf{\textsf{KL}}%
%                             {\lr[#1][]{{#2}\lrmid\|{#3}}}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lrset]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lrset]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lrset]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lrset]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
%\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}

%% overrideable left-right delimeters
% \lr(){foo} -> \left(foo\right)
% \lr[\big](){foo} -> \big({foo}\big)
% \lr[][]{foo} -> \left[{foo}\right]  -- double [] to avoid delims begin processed as opt
% this version should nest correctly
\newcommand\lr[4][]{%
  \ifthenelse{\equal{#1{}}{{}}}%
             {{\left#2\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
             {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
}
% \makeatletter
% \newcommand\lr[4][]{%
%   \ifthenelse{\equal{#1{}}{{}}}%
%              {\def\@lrcontent{#4}%
%                \mathopen{\left#2\vphantom\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
%              {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
% }
% \makeatother

% old version -- use \lrset( \lrset) in place of \left( right).  Cannot be nested!!
\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lrset[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%



==> mdlc_neurips (1)/_fig_4rooms.tex <==
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/4rooms.png}
  %\vspace{-3mm}
  \caption{MDL-C rapidly adapts to new goal locations (top row) and rule changes (bottom row). All curves represent averages taken over 10 random seeds, with the shading indicating standard error.}
  \label{fig:4rooms}
\end{figure*}

==> mdlc_neurips (1)/_fig_dmc.tex <==
\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/dmc_results.pdf}
  %\vspace{-3mm}
  \caption{MDL-C improves both sequential and parallel learning in continuous control tasks. All curves represent averages taken over 8 random seeds, with the shading indicating standard error. In (d), solid curves represent averages over each feature within a category.}
  \label{fig:dmc}
\end{figure*}

==> mdlc_neurips (1)/_fig_schematic.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.65\linewidth]{figures/schematics.pdf} 
\caption{
    \label{fig:schematic}
    \textbf{(A)} Illustration of a generative model of optimal policy parameters. $\hat{w}_1=(1-\beta) w_{11}$ shrinks towards the origin, becoming a closer estimate of $\overline{w}_1$ than $w_{11}$.
    \textbf{(B)} Sparsity-inducing priors over $\beta$.
}
\end{figure}

==> mdlc_neurips (1)/abstract.tex <==
\begin{abstract}
  We propose a novel framework for multitask reinforcement learning based on the \textit{minimum description length} (MDL) principle. In this approach, which we term \textit{MDL-control} (MDL-C), the agent learns the common structure among the tasks with which it is faced and then distills it into a simpler representation which facilitates faster convergence and generalization to new tasks. In doing so, MDL-C naturally balances adaptation to each task with epistemic uncertainty about the task distribution. We motivate MDL-C via formal connections between the MDL principle and Bayesian inference, derive theoretical performance guarantees, and demonstrate MDL-C's empirical effectiveness on both discrete and high-dimensional continuous control tasks. %Empirically, this framework is used to modify existing policy optimization approaches and improves their multitask performance in both discrete and high-dimensional continuous control problems. 
\end{abstract}

==> mdlc_neurips (1)/alg_replay.tex <==
\begin{algorithm}[!t]
	\caption{MDL-C for Sequential Multitask Learning with Persistent Replay}\label{alg:mdlc_replay}
		%\setstretch{1.35}
		\begin{algorithmic}[1] 
		    \STATE require: task distribution $\pr_\mathcal M$, policy class $\Theta$, non-increasing coefficients $\{\eta_{k}\}_{k=1}^K$
		    \STATE initialize: default policy distribution  $\nu_1\in\mathsf{N}\subseteq\mathcal P(\Theta)$, default policy dataset $\mathcal D_0 \gets \emptyset$
			\FOR{tasks $k=1, 2, \dots, K $}
			    \STATE Sample a task $M_k=(\St, \A, \mathsf P_k, r_k, \gamma_k, \rho_k)\sim \mathcal P_\mathcal M(\cdot)$
                \STATE Optimize control policy: 
                \begin{equation} 
                    \theta_k \gets \argmax_{\theta\in\Theta} V^\pi_{M_k} - \alpha \E_{s\sim d^\pi_{\rho_k}}\E_{w\sim\nu_k}\kl[\pi_w(\cdot|s), \pi_\theta(\cdot|s)]
                \end{equation}
                \STATE Add data to default policy replay:
                \begin{equation}
                    \mathcal D_k \gets \mathcal D_{k-1} \cup \{(s_m, \hat\pi_{\theta_k}(s_m))\}_{m=1}^M,
                \end{equation}
                where $M = |\St|$ for finite/small state spaces
                \STATE 
                    Update default policy distribution:
                    \begin{align}
                        \nu_{k+1} \gets \argmin_{\nu \in \mathsf N} \frac{1}{\eta_{k-1}} \kl[\nu(\cdot), p(\cdot)] + \sum_{i=1}^k \sum_{m=1}^M\E_{w\sim\nu}\kl[\hat\pi_{\theta_i}^\star(\cdot|s_m), \pi_w(\cdot|s_m)]
                    \end{align}
                    %\begin{align}
                    %    \nu_{k+1} \gets \argmin_{\nu \in \mathsf N} \kl[\nu(\cdot), p(\cdot)] + \E_{s\sim\mathcal D_k}\E_{w\sim\nu}\kl[\hat\pi_i^\star(\cdot|s), \pi_w(\cdot|s_m)]
                    %\end{align}
                
                %\STATE \textcolor{purple}{Option 2: Add control policy to set:
                %\begin{equation}
                %    \Pi_k^\star \gets \Pi_{k-1} \cup \{\hat\pi_k^\star\}
                %\end{equation}
                %}
			    %\STATE \textcolor{purple}{Update default policy distribution:
                %    \begin{align}
                %        \nu_{k+1} \gets \argmin_{\nu \in \mathsf N} \kl[\nu(\cdot), p(\cdot)] + \E_{w\sim\nu}\kl[\hat\pi_k^\star, \pi_w]
                %    \end{align}
                %}
			 \ENDFOR
	\end{algorithmic}
\end{algorithm}

==> mdlc_neurips (1)/intro.tex <==
\section{Introduction}
In order to learn efficiently in a complex world with multiple,  sometimes rapidly changing objectives, both animals and machines must leverage information obtained from past experience. This is a challenging task, as processing and storing all relevant information is computationally infeasible. How can an intelligent agent address this problem? We hypothesize that one route may lie in the \textit{dual process theory} of cognition, a longstanding framework in cognitive psychology first introduced by William James \citep{james1890principles} which lies at the heart of many dichotomies in both cognitive science and machine learning. Examples include goal-directed versus habitual behavior \citep{Graybiel:2008}, model-based versus model-free reinforcement learning \citep{daw:2011_twostep,Sutton:1998}, and ``System 1'' versus ``System 2'' thinking \citep{kahneman2011thinking}. In each of these paradigms, a complex, ``control'' process trades off with a simple, ``default'' process to guide actions. Why has this been such a successful and enduring conceptual motif? Our hypothesis is that default processes often serve to distill common structure from the tasks consistently faced by animals and agents, facilitating generalization and rapid learning on new objectives. For example, drivers can automatically traverse commonly traveled roads en route to new destinations, and chefs quickly learn new dishes on the back of well-honed fundamental techniques. Importantly, even intricate tasks can become automatic, if repeated often enough (e.g., the combination of fine motor commands required to swing a tennis racket): the default process must be sufficiently expressive to learn common behaviors, regardless of their complexity. In reality, most processes likely lie on a continuum between simplicity and complexity.

In reinforcement learning (RL; \citealp{Sutton:1998}), the problem of improving sample efficiency on new tasks is crucial to the developement of general agents which can learn effectively in the real world \citep{botvinick2015stats,zhang:2021_rlgen}. Intriguingly, one family of approaches which have shown promise in this regard are \textit{regularized policy optimization} algorithms, in which a goal-specific control \textit{policy} is paired with a simple yet general default \textit{policy} to facilitate learning across multiple tasks \citep{Teh:2017_distral,Galashov:2019,Goyal:2020,Goyal:2019,Moskovitz:2021_rpotheory}. One difficulty in algorithm design, however, is how much or how little to constrain the default policy, and in what way. An overly simple default policy will fail to identify and exploit commonalities among tasks, while an overly complex model may overfit to a single task and fail to generalize. Most approaches manually specify an asymmetry between the control and default policies, such as hiding input information \citep{Galashov:2019} or constraining the model class \citep{Lai:2021_compression}. Ideally, we'd like an adaptive approach that can learn the appropriate degree of complexity via experience. 

The \textit{minimum description length principle} (MDL; \citealp{rissanen_78mdl}), which in general holds that one should prefer the simplest model that accurately fits the data, offers a guiding framework for algorithm design that does just that, enabling the default policy to optimally trade off between adapting to information from new tasks and maintaining simplicity. 
%\ted{intuition; driving example etc.}
%Reinforcement learning (RL; \citep{Sutton:1998}) has achieved impressive successes in recent years \citep{Silver:2016,Silver:2017} \ted{DQN, AlphaStar, etc.}. From an engineering perspective, while there are promising steps towards solving real-world problems \ted{cite balloon paper, fusion}, ... From a scientific perspective (what properties of biological intelligence facilitate efficient learning on multiple tasks in natural settings)... One fundamental problem faced by both animals and machines attempting to navigate their environments is how to leverage past experiences to more efficiently complete new tasks. One major obstacle in this endeavor is the world's complexity: there is simply too much information to store it all and reuse. How can an intelligent agent handle this? We hypothesize that one route may lie in the \textit{dual process theory} of cognition a longstanding framework in cognitive psychology first introduced by William James \citep{james1890principles}. Habits/automatic mode distills common structure from the world which can be used to guide future learning. For example, driving 
%RPO methods already embody this, but not necessarily in a principled way. When we've only seen a few tasks, we don't want to overfit and prevent efficient learning on future tasks. The \textit{minimum description length} (MDL; \citep{rissanen_78mdl}) offers a principled framework for this. 
Inspired by dual process theory and the MDL principle, we propose  \textit{MDL-control} (MDL-C, pronounced ``middle-cee''), a principled RPO framework for multitask RL. In \cref{sect:rl_intro}, we formally introduce multitask RL and describe RPO approaches within this setting. In \cref{sec:mdl-principle}, we describe MDL and the variational coding framework, from which we extract MDL-C and derive its formal performance characteristics. In \cref{sect:experiments}, we demonstrate its empirical effectiveness in both discrete and continuous control settings. Finally, we discuss related ideas from the the literature (\cref{sect:related_work}) and conclude (\cref{sect:conclusion}). 
%The primary contributions of this paper are as follows:
%\begin{itemize}
%  \item We propose the \textit{minimum description length control}%(MDL-C, pronounced ``middle-cee'') framework for multitask RL, a principled approach for rapid learning of new tasks. We show that THEORY. 
%  \item We 
%  \item We show it works 
%\end{itemize}



==> mdlc_neurips (1)/m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> mdlc_neurips (1)/m.symbols.tex <==
\RequirePackage{ifthen}
\RequirePackage{mathtools}

% use | for math mode
%\catcode`\|=3


% RL as inference
\newcommand{\opt}{\mathcal{O}}

% pg theory
\newcommand{\J}{\mathcal{J}^{\star}_\lambda}
\newcommand{\Jz}{\mathcal{J}^{\alpha}_\lambda}
\newcommand{\Ju}{\mathcal{J}_\lambda}
\newcommand{\kl}{\mathsf{KL}}
\newcommand{\pitheta}{\pi_{\theta}(a|s)}
\newcommand{\pistar}{\pi^*(a|s)}
\newcommand{\piz}{\pi_0}
\newcommand{\St}{\mathcal S}
\newcommand{\A}{\mathcal A}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\Dinf}{\left\| \frac{d_{\rho}^{\pi^\star} }{\mu}  \right \|_\infty}
\newcommand{\kappaA}{\kappa^\alpha_{\mathcal A}(s)}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\tv}{d_{\mathrm{TV}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathbb E}
\newcommand{\vw}{\vec w}
\newcommand{\prtr}{\mathsf P(s_{h+1}|s_h, a_h)}

% DRL
\newcommand{\Dq}{\stackrel{D}{=}}
\newcommand{\Dqdef}{\stackrel{D}{\coloneqq}}
\newcommand{\bellop}{\mathcal{T}}

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% symbols for probability distributions
\newcommand{\pr}{\mathsf{P}}
%\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
%\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
%\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lrset]{x} -> \mathbb{E}_a \lrset[ x \lrset]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lrset]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lrset]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lrset]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lrset]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
% \newcommand{\angles}[2][\lrset]{{\newlr #1\langle{#2}#1\rangle}}
\newcommand{\angles}[2][]{\lr[#1]\langle\rangle{#2}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lrset]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
%\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
%                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
%\newcommand{\KL}[3][]{\ensuremath{\textbf{\textsf{KL}}%
%                             {\lr[#1][]{{#2}\lrmid\|{#3}}}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lrset]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lrset]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lrset]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lrset]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
%\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}

%% overrideable left-right delimeters
% \lr(){foo} -> \left(foo\right)
% \lr[\big](){foo} -> \big({foo}\big)
% \lr[][]{foo} -> \left[{foo}\right]  -- double [] to avoid delims begin processed as opt
% this version should nest correctly
\newcommand\lr[4][]{%
  \ifthenelse{\equal{#1{}}{{}}}%
             {{\left#2\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
             {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
}
% \makeatletter
% \newcommand\lr[4][]{%
%   \ifthenelse{\equal{#1{}}{{}}}%
%              {\def\@lrcontent{#4}%
%                \mathopen{\left#2\vphantom\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
%              {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
% }
% \makeatother

% old version -- use \lrset( \lrset) in place of \left( right).  Cannot be nested!!
\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lrset[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%



==> mdlc_neurips (1)/multitask_learning_algorithm.tex <==
\begin{algorithm}[!t]
	\caption{Idealized MDL-C for Multitask Learning}\label{alg:mdlc}
		%\setstretch{1.35}
		\begin{algorithmic}[1] 
		    \STATE require: task distribution $\pr_\mathcal M$, policy class $\Pi$, coefficients $\{\eta_{k}\}$
		    \STATE initialize: default policy distribution  $\nu_1\in\mathsf{N}$
			\FOR{tasks $k=1, 2, \dots, K $}
			    \STATE Sample a task $M_k\sim \mathcal P_\mathcal M(\cdot)$
                \STATE Optimize control policy: 
                \begin{equation} 
                    \hat\pi_k^\star = \argmax_{\pi\in\Pi} V^\pi_{M_k} - \lambda \E_{s\sim d^\pi}\E_{w\sim\nu_k}\kl[\pi_w(a|s), \pi(a|s)]
						\label{algo:eq:control}
                \end{equation}
			    \STATE Update default policy distribution:
                    \begin{align}
                        \nu_{k+1} = \argmin_{\nu \in \mathsf N} \kl[\nu, p] + \E_{w\sim\nu}\kl[\hat\pi_k^\star, \pi_w]
						\label{algo:eq:default}
                    \end{align}
			 \ENDFOR
	\end{algorithmic}
\end{algorithm}

==> mdlc_neurips (1)/related_work.tex <==
\section{Related Work} \label{sect:related_work}
    MDL-C can be viewed as an extension of recent approaches to learning default policies (``behavioral priors'') from the optimal policies of related tasks~\citep{Teh:2017_distral, tirumala2020behavior}.
    For a default policy to be useful for transfer learning, it is crucial to balance the ability of the default policy to ``copy'' the control policies with its expressiveness.
    If the default policy is too expressive, it is likely to overfit on past tasks and fail to generalize to unseen tasks.
    Whereas prior work primarily hand-crafts structural constraints into the default policies to avoid overfitting (e.g., by hiding certain state information from the default policy; \citealp{Galashov:2019}), MDL-C learns such a balance from data with sparsity-inducing priors via variational inference. MDL-C may also be derived from the RL-as-inference framework~(\citealp{Levine:2018_rlai}; \Cref{supp:sec:rl_as_inference}).
    MDL-C thus has close connections with algorithms such as MPO~\citep{Abdolmaleki:2018} and VIREL~\citep{Fellows:2020_virel}, discussed in \cref{supp:sec:rl_as_inference}. As a general framework, MDL-C is also connected to the long and well-established literature on choosing appropriate Bayesian priors~\citep{jeffreys_prior46, bernardo2005reference, casella1985introduction}, and more recent work that focuses on learning such priors for large-scale machine learning models~\citep{nalisnick2017learning, nalisnick2021predictive, atanov2018deep}. For a further discussion of related work, particularly concerning the application of MDL to the RL setting, see \cref{sect:more_related}. 
    

    
    
    
% Reinforcement learning as inference
% Learning Bayesian priors

%MDL-C builds upon recent progress in the literature that uses regularized reinforcement learning~\citep{geist2019theory}.



==> mdlc_neurips (1)/stash.tex <==
%
% Like the Jame-Stein estimator, dominates maximum-likelihood estimator~\citepAPP{efron1973stein}.
% %
% Two such choices are
% %
% \begin{enumerate}
%     \item $p(\beta) \propto \beta^{-(a+1)}$ 
%     \item $p(\beta) \propto \exp(-c\beta/2)\beta^{-(a+1)}$ 
% \end{enumerate}
% %
% for $-(d/2 - 2) \leq a < 1$ and $c > 0$.



%
%\subsection{Choices of \texorpdfstring{$p(\beta)$}{} }
%Two such choices are $p(\beta) \propto \beta^{-(1+a)}$ and $p(\beta) \propto \beta^{-(1+a)}\exp(c\sigma^2/2\beta)$, for bounded constants $a$ and $c$.
%Interestingly, these are both priors that encode the belief that the groups of tasks in $\mathcal{M}$ are well separated, or equivalently that $\beta$ is likely to be small.
%
%
%\begin{table}[h!]
%  \begin{center}
%  \begin{tabular}{c c c}
%    $p(\beta)$ & $p(\alpha^2)$ & $p(\theta | \beta, \sigma^2)$\\[0.5em]
%    \hline
%    \hline
%    $1 / \beta$ & Jeffreys & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\beta^{-(1+a)}\exp(c\beta/{2})$ & Inverse-Gamma & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    Half-Cauchy\calvin{To-check} & Half-Cauchy & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\delta(\beta - 1)$ & $\delta(\alpha^2-\sigma^2)$ & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\delta(\beta)$ & $\delta(\alpha^2 -\infty)$ & $\text{Uniform}$
%  \end{tabular}
%  \end{center}
%  \caption{Choices of $p(\beta)$ and the induced prior over $\alpha^2$ and $\theta$.}
%  \label{supp:table:prior_choices}
%  \end{table}

==> stash.tex <==
%
% Like the Jame-Stein estimator, dominates maximum-likelihood estimator~\citepAPP{efron1973stein}.
% %
% Two such choices are
% %
% \begin{enumerate}
%     \item $p(\beta) \propto \beta^{-(a+1)}$ 
%     \item $p(\beta) \propto \exp(-c\beta/2)\beta^{-(a+1)}$ 
% \end{enumerate}
% %
% for $-(d/2 - 2) \leq a < 1$ and $c > 0$.



%
%\subsection{Choices of \texorpdfstring{$p(\beta)$}{} }
%Two such choices are $p(\beta) \propto \beta^{-(1+a)}$ and $p(\beta) \propto \beta^{-(1+a)}\exp(c\sigma^2/2\beta)$, for bounded constants $a$ and $c$.
%Interestingly, these are both priors that encode the belief that the groups of tasks in $\mathcal{M}$ are well separated, or equivalently that $\beta$ is likely to be small.
%
%
%\begin{table}[h!]
%  \begin{center}
%  \begin{tabular}{c c c}
%    $p(\beta)$ & $p(\alpha^2)$ & $p(\theta | \beta, \sigma^2)$\\[0.5em]
%    \hline
%    \hline
%    $1 / \beta$ & Jeffreys & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\beta^{-(1+a)}\exp(c\beta/{2})$ & Inverse-Gamma & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    Half-Cauchy\calvin{To-check} & Half-Cauchy & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\delta(\beta - 1)$ & $\delta(\alpha^2-\sigma^2)$ & $\mathcal{N}(0, \alpha^2)$\\[0.5em]
%    $\delta(\beta)$ & $\delta(\alpha^2 -\infty)$ & $\text{Uniform}$
%  \end{tabular}
%  \end{center}
%  \caption{Choices of $p(\beta)$ and the induced prior over $\alpha^2$ and $\theta$.}
%  \label{supp:table:prior_choices}
%  \end{table}
